A pair of TESS planets spanning the radius valley around the nearby mid-M dwarf LTT 3780

We present the confirmation of two new planets transiting the nearby mid-M dwarf LTT 3780 (TIC 36724087, TOI-732, $V=13.07$, $K_s=8.204$, $R_s$=0.374 R$_{\odot}$, $M_s$=0.401 M$_{\odot}$, d=22 pc). The two planet candidates are identified in a single TESS sector and are validated with reconnaissance spectroscopy, ground-based photometric follow-up, and high-resolution imaging. With measured orbital periods of $P_b=0.77$ days, $P_c=12.25$ days and sizes $r_{p,b}=1.33\pm 0.07$ R$_{\oplus}$, $r_{p,c}=2.30\pm 0.16$ R$_{\oplus}$, the two planets span the radius valley in period-radius space around low mass stars thus making the system a laboratory to test competing theories of the emergence of the radius valley in that stellar mass regime. By combining 63 precise radial-velocity measurements from HARPS and HARPS-N, we measure planet masses of $m_{p,b}=2.62^{+0.48}_{-0.46}$ M$_{\oplus}$ and $m_{p,c}=8.6^{+1.6}_{-1.3}$ M$_{\oplus}$, which indicates that LTT 3780b has a bulk composition consistent with being Earth-like, while LTT 3780c likely hosts an extended H/He envelope. We show that the recovered planetary masses are consistent with predictions from both photoevaporation and from core-powered mass loss models. The brightness and small size of LTT 3780, along with the measured planetary parameters, render LTT 3780b and c as accessible targets for atmospheric characterization of planets within the same planetary system and spanning the radius valley.

==> esmtable_tmp.tex <==
\begin{tabular}{lrrrrrrrrrrr}
\toprule
{} &      P &     rp &         Z &          Teq &         Tday &    Kmag &    Teff &     Rs &     Ms &        ESM &   ESMnorm \\
\midrule
LTT 3780b   &  0.768 &  1.332 &  1.064354 &   892.852458 &   982.137704 &   8.204 &  3331.0 &  0.374 &  0.401 &  13.436062 &  0.463312 \\
LHS 3844b   &  0.463 &  1.303 &  3.988285 &   805.854400 &   886.439840 &   9.145 &  3036.0 &  0.189 &  0.151 &  29.000054 &  1.000002 \\
L 168-9b    &  1.402 &  1.390 &  0.450348 &   981.653764 &  1079.819140 &   7.082 &  3800.0 &  0.600 &  0.620 &   9.906946 &  0.341619 \\
GJ 1132b    &  1.629 &  1.130 &  2.406650 &   585.035999 &   643.539598 &   8.322 &  3270.0 &  0.211 &  0.181 &   9.537957 &  0.328895 \\
L 98-59b    &  2.250 &  0.800 &  0.558827 &   607.410761 &   668.151837 &   7.101 &  3412.0 &  0.310 &  0.310 &   4.127090 &  0.142313 \\
L 98-59c    &  3.690 &  1.350 &  1.591348 &   515.071909 &   566.579100 &   7.101 &  3412.0 &  0.310 &  0.310 &   6.858435 &  0.236498 \\
LTT 1445Ab  &  5.359 &  1.380 &  2.038276 &   435.075983 &   478.583582 &   6.500 &  3335.0 &  0.280 &  0.260 &   6.303129 &  0.217349 \\
TRAPPIST-1b &  1.511 &  1.090 &  6.923273 &   405.637555 &   446.201311 &  10.300 &  2559.0 &  0.120 &  0.080 &   3.974637 &  0.137056 \\
LHS 1140c   &  3.778 &  1.280 &  3.117470 &   434.050258 &   477.455284 &   8.821 &  3216.0 &  0.210 &  0.180 &   3.439983 &  0.118620 \\
LP 791-18b  &  0.948 &  1.120 &  3.599687 &   594.494693 &   653.944163 &  10.644 &  2949.0 &  0.171 &  0.139 &   5.912816 &  0.203890 \\
GJ 1252b    &  0.518 &  1.193 &  0.781175 &  1089.924342 &  1198.916776 &   7.915 &  3458.0 &  0.391 &  0.381 &  16.419351 &  0.566185 \\
\bottomrule
\end{tabular}


==> tesspriors.tex <==
\begin{deluxetable}{lc}
\tabletypesize{\small}
%\tablenum{1}
\tablecaption{\tess{} light curve model parameter priors\label{tab:tesspriors}}
\tablewidth{0pt}
\tablehead{\colhead{Parameter} & \colhead{Prior}}
%\decimalcolnumbers
\startdata
$f_0$ & $\mathcal{N}(0,10)$ \\ 
\multicolumn{2}{c}{\emph{GP hyperparameters}} \\
$\ln{\omega_0}$, [days$^{-1}$] & $\mathcal{N}(0,10)$ \\
$\ln{S_0\omega_0^4}$ & $\mathcal{N}(\ln{\text{var}(\mathbf{f}_{\text{TESS}})},10)$ \\
$\ln{s_{\text{TESS}}^2}$ & $\mathcal{N}(\ln{\text{var}(\mathbf{f}_{\text{TESS}})},10)$ \\
\multicolumn{2}{c}{\emph{Stellar parameters}} \\
$M_s$, [\Msun{]} & $\mathcal{N}(0.401,0.012)$ \\
$R_s$, [\Rsun{]} & $\mathcal{N}(0.373,0.011)$ \\
$u_1$ & $\mathcal{U}(0,1)$ \\
$u_2$ & $\mathcal{U}(0,1)$ \\
\multicolumn{2}{c}{\emph{LTT 3780b parameters}} \\
$\ln{P}_b$, [days] & $\mathcal{N}(\ln{0.768},0.5)$ \\
$T_{0,b}$, [BJD-2,457,000] & $\mathcal{N}(1543.911,0.5)$ \\
$\ln{r_{p,b}}$, [\Rearth{]} & $\mathcal{N}(0.5\cdot \ln(Z_b) + \ln{R_s},1)$\tablenotemark{a} \\
$b_b$ & $\mathcal{U}(0,1+r_{p,b}/R_s)$ \\
\multicolumn{2}{c}{\emph{LTT 3780c parameters}} \\
$\ln{P}_c$, [days] & $\mathcal{N}(\ln{12.254},0.5)$ \\
$T_{0,c}$, [BJD-2,457,000] & $\mathcal{N}(1546.848,0.5)$ \\
$\ln{r_{p,c}}$, [\Rearth{]} & $\mathcal{N}(0.5\cdot \ln(Z_c) + \ln{R_s},1)$\tablenotemark{b} \\
$b_c$ & $\mathcal{U}(0,1+r_{p,c}/R_s)$ \\
$e_c$ & $\mathcal{B}(0.867,3.03)$\tablenotemark{c} \\
$\omega_c$, [rad] & $\mathcal{U}(-\pi,\pi)$ \\
\enddata
\tablecomments{Gaussian distributions are denoted by $\mathcal{N}$ and are
  parameterized by mean and standard deviation values. Uniform distributions
  are denoted by $\mathcal{U}$ and bounded by the specified lower and upper
  limits. Beta distributions are denoted by $\mathcal{B}$ and are parameterized
  by the shape parameters $\alpha$ and $\beta$.}
\tablenotetext{a}{The transit depth of TOI-732.01 reported by the SPOC: $Z_b=1253$ ppm.}
\tablenotetext{b}{The transit depth of TOI-732.02 reported by the SPOC: $Z_b=3417$ ppm.}
\tablenotetext{c}{\citealt{kipping13}.}
\end{deluxetable}


==> tesstable.tex <==
\begin{deluxetable*}{lcc}
\tabletypesize{\small}
\tablecaption{Point estimates of the \tess{} model parameters\label{tab:tess}}
\tablewidth{0pt}
\tablehead{Parameter & \multicolumn{2}{c}{Value}}
\startdata
Baseline flux offset, $f_0$ & \multicolumn{2}{c}{nan} \\
& \multicolumn{2}{c}{\emph{Stellar parameters}} \\
& \multicolumn{2}{c}{\emph{GP hyperparameters}} \\
\emph{Planet parameters} && \\
& \emph{LTT 3780b (TOI-732.01)} & \emph{LTT 3780c (TOI-732.02)} \\
Log orbital period, $\ln{P}$ [days] & $-0.26338\pm 0.00007$ & $2.5058\pm 0.0002$ \\
$P$ [days] & $0.768448^{+0.000055}_{-0.000053}$ & $12.2519^{+0.0028}_{-0.0030}$ \\
Time of mid-transit, $T_0$ [BJD - 2,457,000] & $1543.911\pm 0.001$ & $1546.848\pm 0.001$ \\
Transit depth $Z$ [ppt] & $1.087^{+0.098}_{-0.103}$ & $3.24^{+0.41}_{-0.37}$ \\
Transit duration $D$ [hrs] & $0.805^{+0.049}_{-0.072}$ & $1.75^{+0.37}_{-0.28}$ \\
Scaled semimajor axis, $a/R_s$ & $7.03^{+0.23}_{-0.21}$ & $44.55^{+1.45}_{-1.33}$ \\
Planet-to-star radius ratio, $r_p/R_s$ & $0.0330^{+0.0014}_{-0.0016}$ & $0.0570^{+0.0035}_{-0.0033}$ \\
Impact parameter, $b$ & $0.35^{+0.20}_{-0.23}$ & $0.65^{+0.15}_{-0.36}$ \\
Inclination, $i$ & $87.14^{+1.83}_{-1.68}$ & $89.17^{+0.46}_{-0.19}$ \\
Planet radius, $r_p$ [\Rearth{]} & $1.33^{+0.07}_{-0.08}$ & $2.33^{+0.16}_{-0.15}$ \\
Semimajor axis, $a$ [AU] & $0.01211^{+0.00012}_{-0.00012}$ & $0.07673^{+0.00075}_{-0.00077}$ \\
Insolation, $F$ [F$_{\oplus}$] & $103.21^{+6.44}_{-6.43}$ & $2.57^{+0.16}_{-0.16}$ \\
Equilibrium temperature, $T_{\text{eq}}$ [K] && \\
\hspace{2pt} Bond albedo = 0.0 & $888^{+14}_{-14}$ & $353^{+5}_{-6}$ \\
\hspace{2pt} Bond albedo = 0.3 & $813^{+12}_{-13}$ & $323^{+5}_{-5}$ \\
\enddata
\tablecomments{hi}
\end{deluxetable*}


==> tmp.tex <==
%1656.493768 &     4.365 &   2.070 &    HARPS \\
%1661.467140 &    -3.240 &  1.404 &    HARPS \\
%1802.851053 &    2.572 &  1.023 &    HARPS \\
%1803.846779 &   -5.597 &  1.108 &    HARPS \\
%1805.845559 &    -2.572 &  1.921 &    HARPS \\
%1806.845616 &    -9.207 &  1.204 &    HARPS \\
%1807.846332 &    -5.480 &  1.253 &    HARPS \\
1821.837965 &   -0.959 &   1.310 &    HARPS \\
1831.760260 &   -10.056 &  1.330 &  HARPS-N \\
1836.858657 &    -5.946 &   1.403 &    HARPS \\
%1837.840829 &    0.345 &  1.871 &    HARPS \\
%1838.701497 &     5.550 &  1.383 &  HARPS-N \\
%1838.826242 &    2.691 &  2.095 &    HARPS \\
%1840.765628 &   -5.140 &  1.127 &    HARPS \\
%1848.781285 &     4.312 &  1.265 &    HARPS \\
%1849.762582 &    2.163 &  1.439 &  HARPS-N \\
%1850.705912 &    2.137 &  1.258 &    HARPS \\
%1850.724050 &    -5.750 &  1.879 &  HARPS-N \\
%1851.750951 &     4.726 &  1.299 &  HARPS-N \\
%1851.827971 &    7.427 &  1.283 &    HARPS \\
%1853.720299 &   -2.860 &  1.466 &  HARPS-N \\
%1853.778474 &    -5.550 &  1.227 &    HARPS \\
%1854.711812 &   0.084 &  1.601 &  HARPS-N \\
%1855.710547 &    -3.736 &  1.625 &    HARPS \\
%1859.689968 &     4.664 &  1.594 &  HARPS-N \\
%1860.675920 &   -1.692 &  1.514 &  HARPS-N \\
%1861.748520 &     9.461 &   1.428 &  HARPS-N \\
%1871.831541 &       8.832 &   1.542 &    HARPS \\
%1875.854061 &     5.230 &  1.205 &    HARPS \\
%1876.822307 &    0.511 &  1.474 &    HARPS \\
%1880.709503 &    -4.151 &   1.182 &    HARPS \\
%1881.807656 &    1.054 &  1.347 &    HARPS \\
%1882.615112 &    1.965 &  1.424 &    HARPS \\
%1883.763159 &   -2.397 &    0.793 &    HARPS \\
%1885.591151 &    3.297 &  1.158 &  HARPS-N \\
%1885.663874 &    10.528 &  1.402 &    HARPS \\
%1886.819591 &  -0.267 &   1.495 &    HARPS \\
%1887.565649 &    3.144 &  1.189 &  HARPS-N \\
%1887.603717 &     5.962 &  1.506 &    HARPS \\
%1887.636763 &    0.802 &  0.979 &  HARPS-N \\
%1888.574702 &     3.194 &  1.292 &  HARPS-N \\
%1888.685458 &       6.528 &  2.498 &  HARPS-N \\
%1888.740367 &    7.157 &  1.257 &    HARPS \\
%1889.559157 &     2.542 &  1.823 &  HARPS-N \\
%1890.607456 &    -5.537 &   1.080 &  HARPS-N \\
%1891.640382 &      2.155 &  2.151 &  HARPS-N \\
%1893.735385 &    -9.273 &  1.607 &    HARPS \\
%1898.743675 &     5.458 &  1.253 &    HARPS \\
%1899.575496 &     4.327 &   1.432 &  HARPS-N \\
%1900.659751 &   -1.227 &  1.267 &    HARPS \\
%1901.828901 &     1.786 &  1.423 &    HARPS \\
%1903.736264 &    -7.5890 &  1.139 &    HARPS \\
%1907.497916 &    -8.875 &  0.959 &  HARPS-N \\
%1909.501257 &    0.710 &  1.541 &  HARPS-N \\
%1909.606905 &    2.066 &  1.260 &  HARPS-N \\
%1910.568862 &  -0.181 &  1.376 &  HARPS-N \\
%1910.643712 &    -5.925 &  1.782 &  HARPS-N \\
%1911.606848 &     -5.847 &   2.248 &  HARPS-N \\
%1912.548917 &    1.694 &  1.563 &  HARPS-N \\
%1914.526351 &   -5.379 &   1.229 &  HARPS-N \\
%1920.474272 &    -5.199 &  1.996 &  HARPS-N \\
%1921.545030 &   -0.953 &  1.188 &  HARPS-N \\
%1923.563695 &     1.146 &  1.306 &  HARPS-N \\


==> transit_params_tmp.tex <==
\multicolumn{3}{c}{\emph{Planet parameters}} \\ 
& \emph{LTT 3780b (TOI-732.01)} & \emph{LTT 3780c (TOI-732.02)} \\ 


==> tsmtable_tmp.tex <==
\begin{tabular}{lrrrrrrrrrrr}
\toprule
{} &       P &     rp &      mp &         Z &         Teq &   Jmag &    Teff &     Rs &     Ms &        TSM &   TSMnorm \\
\midrule
LTT 3780c   &  12.250 &  2.300 &   8.590 &  3.173463 &  354.694735 &  9.007 &  3331.0 &  0.374 &  0.401 &  71.494466 &  0.823460 \\
K2-18b      &  32.940 &  2.711 &   8.630 &  2.803718 &  290.187998 &  9.763 &  3505.0 &  0.469 &  0.495 &  42.803774 &  0.493006 \\
GJ 143b     &  35.610 &  2.610 &  22.700 &  1.183402 &  427.083686 &  6.081 &  4640.0 &  0.695 &  0.730 &  53.040741 &  0.610913 \\
HD 119130b  &  16.980 &  2.630 &  24.500 &  0.488517 &  801.536391 &  8.730 &  5725.0 &  1.090 &  1.000 &  11.327706 &  0.130470 \\
HD 15337c   &  17.170 &  2.390 &   8.110 &  0.640596 &  648.114603 &  7.553 &  5125.0 &  0.865 &  0.900 &  56.697379 &  0.653030 \\
K2-266d     &  14.700 &  2.930 &   8.900 &  1.457624 &  538.289314 &  9.611 &  4285.0 &  0.703 &  0.686 &  47.133309 &  0.542873 \\
K2-266e     &  19.480 &  2.730 &  14.300 &  1.265423 &  490.070490 &  9.611 &  4285.0 &  0.703 &  0.686 &  21.265243 &  0.244929 \\
K2-38c      &  10.560 &  2.420 &   9.900 &  0.258044 &  928.866993 &  9.911 &  5757.0 &  1.380 &  2.240 &   9.165936 &  0.105572 \\
Kepler-102e &  16.146 &  2.220 &   8.930 &  0.715978 &  604.474163 &  9.984 &  4909.0 &  0.760 &  0.810 &  16.275284 &  0.187456 \\
Kepler-96b  &  15.240 &  2.670 &   8.460 &  0.574967 &  798.909828 &  9.260 &  5690.0 &  1.020 &  1.000 &  30.607749 &  0.352534 \\
TOI-270d    &  11.380 &  2.130 &   5.480 &  2.636410 &  372.621920 &  9.099 &  3386.0 &  0.380 &  0.400 &  86.822044 &  1.000000 \\
TOI-700c    &  16.050 &  2.630 &   7.636 &  3.290288 &  356.678602 &  9.469 &  3480.0 &  0.420 &  0.416 &  77.508681 &  0.892730 \\
\bottomrule
\end{tabular}

